Quantum Backbone Networks for Hybrid Quantum Dataframe Transmission

To realize a global quantum Internet, there is a need for communication between quantum subnetworks. To accomplish this task, there have been multiple design proposals for a quantum backbone network and quantum subnetworks. In this work, we elaborate on the design that uses entanglement and quantum teleportation to build the quantum backbone between packetized quantum networks. We design a network interface to interconnect packetized quantum networks with entanglement-based quantum backbone networks and, moreover, design a scheme to accomplish data transmission over this hybrid quantum network model. We analyze the use of various implementations of the backbone network, focusing our study on backbone networks that use satellite links to continuously distribute entanglement resources. For feasibility, we analyze various system parameters via simulation to benchmark the performance of the overall network.

==> plots/sat_table_data_2.tex <==
\begin{tabular}{|c|c|c|c|c|} 
\cline{3-5}
\multicolumn{1}{c}{}                                                                     &           & Micius            & Starlink-5197     & Iridium-113        \\ 
\hline
\multicolumn{2}{|c|}{Start date, UTC}                                                                & 28/11/2023, 23:17 & 04/12/2023, 06:44 & 04/12/2023, 05:21  \\ 
\hline
\multicolumn{2}{|c|}{End date, UTC}                                                                  & 28/11/2023, 23:27 & 04/12/2023, 06:56 & 04/12/2023, 05:36  \\ 
\hline
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Max elevation \\angle ($\circ$)\end{tabular}} & Munich    & 87                & 73                & 81                 \\ 
\cline{2-5}
                                                                                         & Nuremberg & 83                & 62                & 83                 \\ 
\hline
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Minimum altitude \\(km)\end{tabular}}         & Munich    & 472               & 565               & 792                \\ 
\cline{2-5}
                                                                                         & Nuremberg & 475               & 604               & 789                \\
\hline
\end{tabular}
